Fast and robust tensor decomposition with applications to dictionary learning

We develop fast spectral algorithms for tensor decomposition that match the robustness guarantees of the best known polynomial-time algorithms for this problem based on the sum-of-squares (SOS) semidefinite programming hierarchy. Our algorithms can decompose a 4-tensor with $n$-dimensional orthonormal components in the presence of error with constant spectral norm (when viewed as an $n^2$-by-$n^2$ matrix). The running time is $n^5$ which is close to linear in the input size $n^4$. We also obtain algorithms with similar running time to learn sparsely-used orthogonal dictionaries even when feature representations have constant relative sparsity and non-independent coordinates. The only previous polynomial-time algorithms to solve these problem are based on solving large semidefinite programs. In contrast, our algorithms are easy to implement directly and are based on spectral projections and tensor-mode rearrangements. Or work is inspired by recent of Hopkins, Schramm, Shi, and Steurer (STOC'16) that shows how fast spectral algorithms can achieve the guarantees of SOS for average-case problems. In this work, we introduce general techniques to capture the guarantees of SOS for worst-case problems.

==> content/overcomplete.tex <==
\subsection{Overcomplete $3$-tensors}
Now we assume that $\|a_i\|=1$, $\sum_i a_i a_i^{\top} \preceq \sigma \cdot \Id_d$ and $\max_{i\neq j} |\iprod{a_i,a_j}| \le \rho$.

\begin{lemma}
    For any unit vector $x \in \R^d$,
    $\Iprod{x^{\otimes 4}, \sum_{i}a_i^{\otimes 3}} \le 1+\rho\sigma^2$ and
    $\Iprod{x^{\otimes 3}, \sum_{i}a_i^{\otimes 4}} \le 1+\rho^2\sigma^2$.

    On the other hand, $\sum_i a_i^{\otimes 4}$ has at least one eigenvalue of magnitude at least $n/d$.
\end{lemma}
\begin{proof}
    We reduce the case of $3$-tensors to $4$-tensors.
    By Cauchy-Schwarz,
    \begin{align*}
	\Iprod{x^{\otimes 3}, \sum_{i}a_i^{\otimes 3}}^2
	&\le \|x\|^2\cdot \sum_{i,j} \iprod{a_i,a_j} \iprod{x,a_i}^2\iprod{x,a_j}^2\\
	&\le \sum_{i,j} \Abs{\iprod{a_i,a_j}}\cdot \iprod{x,a_i}^2\iprod{x,a_j}^2
	\intertext{and because $\max_{i\neq j}\Abs{\iprod{a_i,a_j}}\le \rho$,}
	&\le (1-\rho)\sum_{i}  \iprod{x,a_i}^4 +\rho\sum_{i,j} \iprod{x,a_i}^2 \iprod{x,a_j}^2  \\
	&\le (1-\rho)\Iprod{x^{\otimes 4},\sum_i a_i^{\otimes 4}} +\left\| \rho \left(\sum_i a_i a_i^{\top}\right)^{\otimes 2}\right\|\\
	&\le (1-\rho)\Iprod{x^{\otimes 4},\sum_i a_i^{\otimes 4}} + \rho \sigma^2\mper
    \end{align*}
    Now for $4$-tensors, again by Cauchy-Schwarz,
    \begin{align*}
	\Iprod{x^{\otimes 4}, \sum_{i}a_i^{\otimes 4}}^2
	&\le \|x\|^8 \cdot \sum_{i,j} \iprod{a_i,a_j}^2\cdot \iprod{x,a_i}^2 \cdot \iprod{x,a_j}^2\\
	&\le (1-\rho^2)\Iprod{x^{\otimes 4},\sum_{i} a_i^{\otimes 4}}  +  \Iprod{x^{\otimes 4}, \rho^2 \sum_{i,j} a_i a_i^{\top} \otimes a_j a_j^{\top}}\\
	&\le (1-\rho^2)\Iprod{x^{\otimes 4},\sum_{i} a_i^{\otimes 4}}  +  \rho^2 \sigma^2\mper
    \end{align*}
    This concludes the proof of the first two claims.


    To see the second claim, consider the test vector $\sum_i a_i^{\otimes 2}$.
    By assumption, $\sum_i a_i^{\otimes 2} = \sigma \Id_d$, and so $\Norm{\sum_i a_i^{\otimes 2}}_F^2 = \sigma^2 d$.
    On the other hand, if we use $\sum_i a_i^{\otimes 2}$ as a test vector,
    \begin{align*}
	\Iprod{\left(\sum_k a_k^{\otimes 2}\right)\left(\sum_j a_j^{\otimes 2}\right)^\top,\sum_i a_i^{\otimes 4}}
	= \sum_{i,j,k} \iprod{a_i,a_j}^2 \iprod{a_i,a_k}^2
	= \sum_j \Iprod{a_ja_j^{\top}, \sigma\cdot \Id}^2
	= \sigma^2 n.
    \end{align*}
    Thus, dividing by the squared Frobenius norm of the test vector, we have the desired result.
\end{proof}


\begin{lemma}
Suppose we are given
    \[
	T = \sum_i a_i^{\otimes 3} + E
    \]
\end{lemma}
\begin{proof}
    Let $g \sim \cN(0,\Id_d)$.
    Let $S = \sum_{i<n} a_i^{\otimes 3}$, and let $T = a_n^{\otimes 3} + S + E$, where $E$ is an error matrix.
    We want to bound the spectral norm of
    \begin{align*}
	\Tr_{\R^d}((g^{\top} T_{\{1\}\{23\}}\otimes \Id_d \otimes \Id_d)(T \otimes T))
	&= \sum_{ijk}g_i \cdot \iprod{\row_i(T),e_j \otimes e_k} \cdot T_j \otimes T_k\\
	&= \sum_{i}g_i \left(\sum_{jk} T_{ijk} \cdot T_j \otimes T_k\right)\mper
    \end{align*}
    Using \pref{lem:gflat}, the spectral norm of this matrix is with high probability bounded by the spectral norm of the $d^3 \times d^2$ matrices
    \[
	\max\left\{ \left\|\left((T\otimes \Id_{d^2})(T\otimes T)\right)_{\{123\}\{45\}}\right\|,\left\|\left((T\otimes \Id_{d^2})(T\otimes T)\right)_{\{125\}\{43\}}\right\|\right\},
    \]
or the matrices whose $i$th $d^2 \times d^2$ block are $\sum_{jk} T_{ijk} \cdot T_j \otimes T_k$ and $\sum_{jk} T_{ijk} \cdot T_j^{\top} \otimes T_k^{\top}$, respectively.

We first restrict our attention to the $S$ component of $T$.
    \begin{align*}
	\left((S\otimes \Id_{d^2})(S\otimes S)\right)_{\{123\}\{45\}}
	&= \sum_{ijk} \iprod{a_i,a_j}\iprod{a_i,a_k} (a_i \otimes a_j \otimes a_k)(a_j \otimes a_k)^{\top}\mper
    \end{align*}
    When $i = j = k$, we have that this term is just
    \[
	\|\sum_{i} a_i^{\otimes 5} \|^2 \le \|\sum_i a_i^{\otimes 4}\|\cdot \|\sum_i a_i^{\otimes 6}\|.
    \]
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

    When $i$ is equal to neither $j$ nor $k$, $i \neq j,k$, then for any unit vectors $u \in \R^{d^3},v \in \R^{d^2}$,
    \begin{align*}
	&\left(\sum_{i\neq j,k} \iprod{a_i,a_j}\iprod{a_i,a_k} \iprod{u,(a_i \otimes a_j \otimes a_k)}\iprod{v,(a_j \otimes a_k)}\right)^2\\
	&\le \left(\sum_{i\neq j, k} \iprod{a_i,a_j}^2\iprod{u,(a_i \otimes a_j \otimes a_k)}^2\right)
	\left(\sum_{i\neq j, k} \iprod{a_i,a_k}^2 \iprod{v,(a_j \otimes a_k)}^2\right)\\
	&\le \left\|\rho^2 \left(\sum_{i} a_i a_i^{\top}\right)^{\otimes 3}\right\|\cdot
	\left\|\left(\sum_{k} a_k^{\top} \left(\sum_i a_i a_i^{\top}\right)a_k \cdot a_k a_k^{\top} \right) \otimes \left(\sum_j a_j^{\otimes 4}\right)\right\|\\
	&\le \rho^2\sigma^3 \cdot \sigma^2 \cdot \|\sum_j a_j^{\otimes 4}\|\mper
    \end{align*}
    So the contribution of these terms is at most $\rho \sigma^{5/2} \|\sum_j a_j^{\otimes 4}\|^{1/2}$.

    When $i$ is equal to exactly one of $j,k$, say $i = j \neq k$, then for any unit vectors $u \in \R^{d^3},v\in \R^{d^2}$,
    \begin{align*}
	\left(\sum_{i\neq k} \iprod{a_i,a_k} \iprod{u,(a_i \otimes a_i \otimes a_k)}\iprod{v,(a_i \otimes a_k)}\right)^2
	&\le \left\|\sum_{i\neq k}\iprod{a_i,a_k}^2\cdot a_i^{\otimes 4}\otimes a_k^{\otimes 2}\right\|\cdot \left\|\sum_{i\neq k}a_ia_i^{\top} \otimes a_k a_k^{\top}\right\|\\
	&\le \rho^2 \sigma \left\|\sum_{i} a_i^{\otimes 4}\right\|\cdot \sigma^2\mper
    \end{align*}
    Thus the contribution of these terms is bounded by $\rho\sigma^{3/2}\|\sum_i a_i^{\otimes 4}\|^{1/2}$.

    Thus the spectral norm of this matrix is at most
    \[
	\left\|\sum_i a_i^{\otimes 4}\right\|^{1/2} \cdot \left(\left\|\sum_i a_i^{\otimes 6}\right\|^{1/2} + \rho\sigma^{3/2} + \rho\sigma^{5/2}\right)\mper
    \]

\end{proof}
